Hamiltonian engineering with time-ordered evolution for unitary control of electron spins in semiconductor quantum dots

We present a unitary control pulse design method for a scalable quantum computer architecture based on electron spins in lateral quantum dots. We employ simultaneous control of spin interactions and derive the functional forms of spin Hamiltonian parameter pulses for a universal set of 1- and 2-qubit logic gates. This includes selective spin rotations with the weak local g-factor variations in the presence of the global oscillating field, and a Control-Phase operation with the simultaneous control of g-factors and exchange couplings. We outline how to generalize the control scheme to multiqubit gate operations and the case of constrained or imperfect control of the Hamiltonian parameters.

==> generalization.tex <==
\section{Scalability and generalizations of the control scheme}

A few lines here
The goal of this subsection are


\subsection{Numerical design of a 3-qubit Control-SWAP gate}

Procedure: have several quantum gates in a circuit. 
Optimization over control amplitudes $A_i, B_i, C_i$. 

Few-parameter GRAPE. 


